Fast joint detection-estimation of evoked brain activity in event-related fMRI using a variational approach

In standard clinical within-subject analyses of event-related fMRI data, two steps are usually performed separately: detection of brain activity and estimation of the hemodynamic response. Because these two steps are inherently linked, we adopt the so-called region-based Joint Detection-Estimation (JDE) framework that addresses this joint issue using a multivariate inference for detection and estimation. JDE is built by making use of a regional bilinear generative model of the BOLD response and constraining the parameter estimation by physiological priors using temporal and spatial information in a Markovian modeling. In contrast to previous works that use Markov Chain Monte Carlo (MCMC) techniques to approximate the resulting intractable posterior distribution, we recast the JDE into a missing data framework and derive a Variational Expectation-Maximization (VEM) algorithm for its inference. A variational approximation is used to approximate the Markovian model in the unsupervised spatially adaptive JDE inference, which allows fine automatic tuning of spatial regularisation parameters. It follows a new algorithm that exhibits interesting properties compared to the previously used MCMC-based approach. Experiments on artificial and real data show that VEM-JDE is robust to model mis-specification and provides computational gain while maintaining good performance in terms of activation detection and hemodynamic shape recovery.

==> abrege.tex <==
% TEX 7(ascii) bits
%
% ABREGE.tex
% LaTeX document
% Author: J.I./P.C. 
% Date  : Juillet 1996
%
% Raccourcis d'expressions tr\`es usit\'ees
%
% Derniere modif le 03-2000
%

% Raccourci pour \XS
\def\XS{\xspace}

%%%%%%%%%%%%%%%%%%% Pour definir nouvelle commande de changement de taille
\RequirePackage{ifthen}
\RequirePackage{calc}
\RequirePackage{xspace}

\def\gui#1{<<\,#1\,>>}
\def\<{\og}
\def\>{\fg}

\newcommand{\taille}[1][\scad]{%
\ifthenelse{#1 = -5}{}{}%
\ifthenelse{#1 = -4}{\tiny}{}%
\ifthenelse{#1 = -3}{\scriptsize}{}%
\ifthenelse{#1 = -2}{\footnotesize}{}%
\ifthenelse{#1 = -1}{\small}{}%
\ifthenelse{#1 = 0}{\normalsize}{}%
\ifthenelse{#1 = 1}{\large}{}%
\ifthenelse{#1 = 2}{\Large}{}%
\ifthenelse{#1 = 3}{\LARGE}{}%
\ifthenelse{#1 = 4}{\huge}{}%
\ifthenelse{#1 = 5}{\Huge}{}}

\newboolean{@serif}
\setboolean{@serif}{true}
\def\scad{-5} % scadefaultsize

\newcounter{taille}
\newcommand{\sca}[2][\scad]{\setcounter{taille}{#1}%
  \ifthenelse{\boolean{@serif}}
  {{\taille[\thetaille]\textsc{#2}}}
  {\setcounter{taille}{\value{taille}-1}{\uppercase{\taille[\thetaille]#2}}}}

% Mise en commentaire rapide !
\def\rem#1{}                    % rem{bla bla bla}

% References automatiquement entre parenthese
\def\reff#1{\XS(\ref{#1})}
\def\refs#1{section~\ref{#1}}
\def\refS#1{Section~\ref{#1}}

\newcommand{\clearemptydoublepage}{\newpage{\pagestyle{empty}\cleardoublepage}}  
% Num\'ero (pour biblio)
\def\numero{n\'e}
\def\Numero{N\'e}
\def\ier{$^{\text{\small er}}$\XS}
\def\iere{$^{\text{\small re}}$\XS}
\def\ieme{$^{\text{\small e}}$\XS}

% Majuscules
\def\UP#1{\uppercase{#1}}       % majuscules
\def\up#1{\uppercase{#1}}       % majuscules

% Liste des abreges
\def\adhoc{\textit{ad hoc}\XS}
\def\apost{\textit{a posteriori}\XS}
\def\aPost{\textit{a Posteriori}\XS}
\def\Apost{\textit{A Posteriori}\XS}
\def\map{\textsc{map}\XS}
\def\eap{\textsc{eap}\XS}
\def\post{\textit{posterior}\XS}
\def\Post{\textit{Posterior}\XS}
\def\afortio{\textit{a fortiori}\XS}
\def\Afortio{\textit{A fortiori}\XS}
\def\aprio{\textit{a priori}\XS}
\def\acont{\textit{a contrario}\XS}
\def\Aprio{\textit{A priori}\XS}
\def\Cad{C'est-\`a-dire\XS}
\def\cad{c'est-\`a-dire\XS}
\def\cf{\textit{cf.}\XS}
\def\cv{\textit{curriculum vit\ae}\XS}
\def\Cv{\textit{Curriculum vit\ae}\XS}
\def\CV{\textit{Curriculum Vit\ae}\XS}
\def\eg{\textit{e.g.,}\XS}
\def\etal{\textit{et al.}\XS}
\def\etc{\textit{etc\dots}\XS}
\def\etcoll{{\textit et coll.}\XS}
\def\idem{\textit{idem}\XS}
\def\ie{\textit{i.e.,}\XS}
\def\IFF{\textit{if and only if}\XS}
\def\iid{\textit{i.i.d.}\XS}
\def\infine{\textit{in fine}\XS}
\def\insit{\textit{in situ}\XS}
\def\inviv{\textit{in vivo}\XS}
\def\oeuvre{{\oe}uvre\XS}
\def\oeuvres{{\oe}uvres\XS}
\def\recto{\textit{recto}\XS}
\def\Toeplitz{T{\oe}plitz\XS}
\def\vav{vis-\`a-vis\XS}
\def\via{\textit{via}\XS}
\def\vic{\textit{vice-versa}\XS}
\def\verso{\textit{verso}\XS}
%\def\vitae{\textit{vit\ae}\XS}
\def\vs{\textit{vs}\XS}
\def\versus{\textit{versus}\XS}
\def\ssi{\textit{si et seulement si}\XS}
\def\strsen{\textit{stricto sensu}\XS}
\def\wrt{w.r.t.\XS}
\newcommand{\anr}[1][\scad]{\sca[#1]{anr}\XS}
\newcommand{\optimed}[1][\scad]{\sca[#1]{optimed}\XS}

% Algorithmes et m\'ethodes
\newcommand{\art}[1][\scad]{\sca[#1]{art}\XS}
\newcommand{\cnd}[1][\scad]{\sca[#1]{cnd}\XS}
\newcommand{\ndt}[1][\scad]{\sca[#1]{ndt}\XS}
\newcommand{\gnc}[1][\scad]{\sca[#1]{gnc}\XS}
\newcommand{\gnd}[1][\scad]{\sca[#1]{gnd}\XS}
\newcommand{\mfa}[1][\scad]{\sca[#1]{mfa}\XS}
\newcommand{\exmax}[1][\scad]{\sca[#1]{em}\XS}
\def\MCMC{m\'ethodes de \textsc{Monte-Carlo} par Cha\^ines de \textsc{Markov}\XS}
\newcommand{\mcmc}[1][\scad]{\sca[#1]{mcmc}\XS}
\newcommand{\icm}[1][\scad]{\sca[#1]{icm}\XS}
\newcommand{\icd}[1][\scad]{\sca[#1]{icd}\XS}
% Les methodes en ICF
\newcommand{\stmap}[1][\scad]{\sca[#1]{st-map}\XS}
\def\SPM{Statistical Parametric Mapping\XS}
\newcommand{\spm}[1][\scad]{\sca[#1]{spm}\XS}
\def\CSM{Cortical Surface Mapping\XS}
\newcommand{\csm}[1][\scad]{\sca[#1]{csm}\XS}

\newcommand{\anat}{\emph{Anatomist}\XS}
\newcommand{\ala}{\emph{Aladin}\XS}
\def\ALA{AnaLyser Autrement les Donn\'ees d'Imagerie Neurofonctionnelle\XS}
\newcommand{\brst}{\emph{Brainstorm}\XS}
\newcommand{\brv}{\texttt{BrainVISA}\XS}
\newcommand{\spmn}[1][\scad]{\sca[#1]{spm}~{\footnotesize 99}\XS}
\newcommand{\pe}[1][\scad]{\sca[#1]{pe}\XS}
\def\SQUID{Superconducting Quantum Interference Device}
\newcommand{\squid}[1][\scad]{\sca[#1]{squid}\XS}
\def\MEF{M\'ethode des \'El\'ements Finis\XS}
\newcommand{\mef}[1][\scad]{\sca[#1]{mef}\XS}
\def\LCR{liquide C\'ephalo-Rachidien\XS}
\newcommand{\aic}[1][\scad]{\sca[#1]{aic}\XS}
\newcommand{\mdl}[1][\scad]{\sca[#1]{mdl}\XS}
\newcommand{\loreta}[1][\scad]{\sca[#1]{loreta}\XS}
\newcommand{\besa}[1][\scad]{\sca[#1]{besa}\XS}
\newcommand{\mits}[1][\scad]{\sca[#1]{mit}\XS}
\newcommand{\lcr}[1][\scad]{\sca[#1]{lcr}\XS}
\newcommand{\frh}[1][\scad]{\sca[#1]{frh}\XS}
\newcommand{\music}[1][\scad]{\sca[#1]{music}\XS}
\newcommand{\rmus}[1][\scad]{\sca[#1]{rmus}\XS}
\newcommand{\rapm}[1][\scad]{\sca[#1]{rapm}\XS}
\newcommand{\irls}[1][\scad]{\sca[#1]{irls}\XS}

\newcommand{\rsb}[1][\scad]{\sca[#1]{rsb}\XS}
\newcommand{\snr}[1][\scad]{\sca[#1]{snr}\XS}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newcommand{\dess}[1][\scad]{\sca[#1]{DESS}\XS}
%\newcommand{\dea}[1][\scad]{\sca[#1]{DEA}\XS}
%\newcommand{\deug}[1][\scad]{\sca[#1]{DEUG}\XS}
%\newcommand{\deust}[1][\scad]{\sca[#1]{DEUST}\XS}
%\newcommand{\iut}[1][\scad]{\sca[#1]{IUT}\XS}
%\newcommand{\iup}[1][\scad]{\sca[#1]{IUP}\XS}

%%%%%%%%%% Diplomes universitaires
\newcommand{\dess}[1][\scad]{\sca[#1]{dess}\XS}
\newcommand{\dea}[1][\scad]{\sca[#1]{dea}\XS}
\newcommand{\deug}[1][\scad]{\sca[#1]{deug}\XS}
\newcommand{\deust}[1][\scad]{\sca[#1]{deust}\XS}
\newcommand{\iut}[1][\scad]{\sca[#1]{iut}\XS}
\newcommand{\iup}[1][\scad]{\sca[#1]{iup}\XS}

%%%%%%%%%% Filieres universitaires
\newcommand{\eea}[1][\scad]{\sca[#1]{eea}\XS}
\def\EEA{\'Electronique \'Electrotechnique Automatique\XS}
\newcommand{\ats}[1][\scad]{\sca[#1]{ats}\XS}
\def\ATS{Automatique et Traitement du Signal\XS}
\def\ts{traitement du signal\XS}
\def\TS{Traitement du Signal\XS}

%%%%%%%%%% Enseignements 
\newcommand{\te}[1][\scad]{\sca[#1]{te}\XS}
\def\TE{travaux d'\'etudes\XS}
\newcommand{\td}[1][\scad]{\sca[#1]{td}\XS}
\def\TD{travaux dirig\'es\XS}
\newcommand{\tp}[1][\scad]{\sca[#1]{tp}\XS}
\def\TP{travaux pratiques\XS}
\def\TDAO{travaux dirig\'es assist\'es sur ordinateur\XS}
\newcommand{\tdao}[1][\scad]{\sca[#1]{tdao}\XS}

\newcommand{\gbm}[1][\scad]{\sca[#1]{gbm}\XS}
\def\ICF{Imagerie C\'er\'ebrale Fonctionnelle\XS}
\newcommand{\icf}[1][\scad]{\sca[#1]{icf}\XS}

%%%%%%%%%% Modalites ICF en extensif 
\def\EEG{\'Electroenc\'ephalographie\XS}
\def\ECOG{\'Electrocorticogramme\XS}
\def\MEG{Magn\'etoenc\'ephalographie\XS}
\def\MEEG{Magn\'eto/\'Electroenc\'ephalographie\XS}
\def\IRM{Imagerie par R\'esonance Magn\'etique\XS}
\def\IRMf{Imagerie par R\'esonance Magn\'etique fonctionnelle\XS}
%\def\BOLDS{Blood Oxygenated Level Dependent\XS}
\def\BOLD{\emph{Blood-Oxygen-Level Dependent}\xspace}
\def\IRMD{Imagerie par R\'esonance Magn\'etique de Diffusion\XS}
\def\TEMP{Tomographie d'\'Emission Monophotonique\XS}
\def\SPECT{Single Photon Emission Tomography\XS}
\def\TEP{Tomographie par \'Emission de Positons\XS}
\def\PET{Positron Emission Tomography\XS}
\def\DSCr{D\'ebit Sanguin C\'er\'ebral r\'egional\XS}
\def\NIRS{\emph{Near Infra Read Spectroscopy}\XS}
\def\FRH{\emph{Fonction de R\'eponse H\'emodynamique}\XS}

%%%%%%%%%% Modalites ICF en abrege 
\newcommand{\eeg}[1][\scad]{\sca[#1]{eeg}\XS}
\newcommand{\ecog}[1][\scad]{\sca[#1]{ecog}\XS}
\newcommand{\meg}[1][\scad]{\sca[#1]{meg}\XS}
\newcommand{\meeg}[1][\scad]{\sca[#1]{meeg}\XS}
\newcommand{\irmf}[1][\scad]{\sca[#1]{irm}f\XS}
\newcommand{\bolds}[1][\scad]{\sca[#1]{bold}\XS}
\newcommand{\irmd}[1][\scad]{\sca[#1]{irm} de diffusion\XS}
\newcommand{\irm}[1][\scad]{\sca[#1]{irm}\XS}
\newcommand{\rmn}[1][\scad]{\sca[#1]{rmn}\XS}
\newcommand{\temp}[1][\scad]{\sca[#1]{tesp}\XS}
\newcommand{\spect}[1][\scad]{\sca[#1]{spect}\XS}
\newcommand{\tep}[1][\scad]{\sca[#1]{tep}\XS}
\newcommand{\pet}[1][\scad]{\sca[#1]{pet}\XS}
\newcommand{\dscr}[1][\scad]{\sca[#1]{dsc}r\XS}


%%%%%%%%%% Ordinateur 
\newcommand{\pc}[1][\scad]{\sca[#1]{pc}\XS}
%%%%%%%%%% Operating Systemes 
\newcommand{\linux}[1][\scad]{\sca[#1]{Linux}\XS}
\newcommand{\unix}[1][\scad]{\sca[#1]{Unix}\XS}
\newcommand{\msdos}[1][\scad]{\sca[#1]{msdos}\XS}
\newcommand{\sunos}[1][\scad]{\sca[#1]{Sunos}\XS}
\newcommand{\vax}[1][\scad]{\sca[#1]{Vax}\XS}
\newcommand{\hupux}[1][\scad]{\sca[#1]{hp-ux}\XS}
\newcommand{\vms}[1][\scad]{\sca[#1]{vms}\XS}
\newcommand{\solaris}[1][\scad]{\sca[#1]{Solaris}\XS}
\newcommand{\winnt}[1][\scad]{\sca[#1]{Windows-nt}\XS}
\newcommand{\vmware}[1][\scad]{\sca[#1]{vmware}\XS}
\newcommand{\win}[1][\scad]{\sca[#1]{Windows}\XS}

%%%%%%%%%% Calcul scientifique
\newcommand{\labview}[1][\scad]{\sca[#1]{Labview}\XS}
\newcommand{\matlab}[1][\scad]{\sca[#1]{Matlab}\XS}
\newcommand{\simulink}[1][\scad]{\sca[#1]{Simulink}\XS}
\newcommand{\maple}[1][\scad]{\sca[#1]{Maple}\XS}
\newcommand{\mathe}[1][\scad]{\sca[#1]{Mathematica}\XS}
\newcommand{\idl}[1][\scad]{\sca[#1]{Idl}\XS}
\newcommand{\word}[1][\scad]{\sca[#1]{Word 97}\XS}
\newcommand{\excel}[1][\scad]{\sca[#1]{Excel 97}\XS}
\newcommand{\xfig}[1][\scad]{\sca[#1]{Xfig}\XS}
\newcommand{\perf}[1][\scad]{\sca[#1]{\textsf{perforce}}\XS}

%%%%%%%%%% langages
\newcommand{\cmex}[1][\scad]{\sca[#1]{Cmex}\XS}
\newcommand{\pascal}[1][\scad]{\sca[#1]{Pascal}\XS}
\newcommand{\java}[1][\scad]{\sca[#1]{Java}\XS}
\newcommand{\lisp}[1][\scad]{\sca[#1]{Lisp}\XS}
\newcommand{\forts}[1][\scad]{\sca[#1]{Fortran}{\footnotesize 77}\XS}
\newcommand{\fortq}[1][\scad]{\sca[#1]{Fortran}{\footnotesize 90}\XS}
\newcommand{\ada}[1][\scad]{\sca[#1]{Ada}\XS}
\newcommand{\eiffel}[1][\scad]{\sca[#1]{Eiffel}\XS}
\newcommand{\tcsh}[1][\scad]{\sca[#1]{tcsh}\XS}
\newcommand{\ksh}[1][\scad]{\sca[#1]{ksh}\XS}
\newcommand{\bash}[1][\scad]{\sca[#1]{bash}\XS}
\newcommand{\lgc}[1][\scad]{\sca[#1]{C}\XS}
\newcommand{\cpp}[1][\scad]{\sca[#1]{C}\raisebox{.05cm}{{\footnotesize ++}}\XS}
\def\STL{\emph{Standard Template Library}\XS}

% editeurs
\newcommand{\nedit}[1][\scad]{\sca[#1]{\textsf{nedit}}\XS}
\newcommand{\emacs}[1][\scad]{\sca[#1]{\textsf{emacs}}\XS}
\newcommand{\xemacs}[1][\scad]{\sca[#1]{\textsf{xemacs}}\XS}

\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
				T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}

\def\crec{charg\'e de recherches\XS}
\def\Crec{Charg\'e de recherches\XS}
\def\dr{directeur de recherches\XS}
\def\Dr{Directeur de recherches\XS}
\def\Dri{Directrice de recherches\XS}
\def\dri{directrice de recherches\XS}


% congres
\newcommand{\gretsi}[1][\scad]{\sca[#1]{gretsi}\XS}
\newcommand{\maxent}[1][\scad]{\sca[#1]{maxent}\XS}
\newcommand{\icip}[1][\scad]{\sca[#1]{icip}\XS}
\newcommand{\isbi}[1][\scad]{\sca[#1]{isbi}\XS}
\newcommand{\icassp}[1][\scad]{\sca[#1]{icassp}\XS}
\newcommand{\spie}[1][\scad]{\sca[#1]{spie}\XS}
\newcommand{\gdr}[1][\scad]{\sca[#1]{gdr--prc~isis}\XS}
\newcommand{\gt}[1][\scad]{\sca[#1]{gt}\XS}
\newcommand{\rfia}[1][\scad]{\sca[#1]{rfia}\XS}
\newcommand{\eusipco}[1][\scad]{\sca[#1]{eusipco}\XS}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Ajout de famouss.tex
% modif le 25/5/2000 Phiphi
% GPInuts - Famous people - VIP ....
%
\newcommand{\beaunom}[4][0]{{\taille[#1]#2 \uppercase{#3}}%
{\sca[#1]{#4}}\XS}

%\newcommand{\MA}[1][\scad]{{\taille[#1]Marc \uppercase{A}}% 
%{\sca[#1]{llain}\XS}}
\newcommand{\AlA}[1][\scad]{\beaunom[#1]{Alexandre}{A}{ndrade}}
\newcommand{\AB}[1][\scad]{\beaunom[#1]{Amandine}{B}{lanc}}
\newcommand{\ABF}[1][\scad]{\beaunom[#1]{Amandine}{B}{lanc~--~Fusco}}
\newcommand{\ACC}[1][\scad]{\beaunom[#1]{Anne--Claire}{C}{roiz\'e}}
\newcommand{\AnD}[1][\scad]{\beaunom[#1]{Antoine}{D}{ucorps}}
\newcommand{\AH}[1][\scad]{\beaunom[#1]{Alain}{H}{erment}}
\newcommand{\AlR}[1][\scad]{\beaunom[#1]{Alexis}{R}{oche}}
\newcommand{\AMD}[1][\scad]{\beaunom[#1]{Ali}{M}{ohammad--Djafari}}
\newcommand{\AR}[1][\scad]{\beaunom[#1]{Andrea}{R}{idolfi}}
\newcommand{\BR}[1][\scad]{\beaunom[#1]{Bernard}{R}{enault}}
\newcommand{\BT}[1][\scad]{\beaunom[#1]{Bruno}{T}{orresani}}
\newcommand{\BeT}[1][\scad]{\beaunom[#1]{Bertrand}{T}{hirion}}
\newcommand{\CH}[1][\scad]{\beaunom[#1]{Christian}{H}{einrich}}
\newcommand{\ChP}[1][\scad]{\beaunom[#1]{Christophe}{P}{allier}}
\newcommand{\ChV}[1][\scad]{\beaunom[#1]{Christophe}{V}{ignat}}
\newcommand{\CP}[1][\scad]{\beaunom[#1]{Cyril}{P}{oupon}}
\newcommand{\CR}[1][\scad]{\beaunom[#1]{Christian}{R}{obert}}
\newcommand{\CS}[1][\scad]{\beaunom[#1]{Charles}{S}{oussen}}
\newcommand{\CVG}[1][\scad]{\beaunom[#1]{Christophe}{V}{ignat}}
\newcommand{\DLB}[1][\scad]{\beaunom[#1]{Denis}{L}{e Bihan}}
\newcommand{\DM}[1][\scad]{\beaunom[#1]{Daniel}{M}{uller}}
\newcommand{\DP}[1][\scad]{\beaunom[#1]{Dimitri}{P}{apadopoulos}}
\newcommand{\DR}[1][\scad]{\beaunom[#1]{Denis}{R}{ivi\'ere}}
\newcommand{\DS}[1][\scad]{\beaunom[#1]{Denis}{S}{chwartz}}
\newcommand{\EM}[1][\scad]{\beaunom[#1]{Eric}{M}{oulines}}
\newcommand{\EDU}[1][\scad]{\beaunom[#1]{Edouard}{D}{uchesnay}}
\newcommand{\FC}[1][\scad]{\beaunom[#1]{Fr\'ed\'eric}{C}{hampagnat}}
\newcommand{\FK}[1][\scad]{\beaunom[#1]{Ferath}{K}{herif}}
\newcommand{\FL}[1][\scad]{\beaunom[#1]{Franck}{L}{etimonier}}
\newcommand{\FV}[1][\scad]{\beaunom[#1]{Francisco}{V}{arela}}
\newcommand{\FDU}[1][\scad]{\beaunom[#1]{Fr\'ed\'eric}{D}{ublanchet}}
\newcommand{\GA}[1][\scad]{\beaunom[#1]{Gilles}{A}{ubert}}
\newcommand{\GDE}[1][\scad]{\beaunom[#1]{Guy}{D}{emoment}}
\newcommand{\GF}[1][\scad]{\beaunom[#1]{Guillaume}{F}{landin}}
\newcommand{\GLB}[1][\scad]{\beaunom[#1]{Guy Le}{B}{esnerais}}
\newcommand{\GM}[1][\scad]{\beaunom[#1]{Guillaume}{M}{arrelec}}
\newcommand{\HB}[1][\scad]{\beaunom[#1]{Habib}{B}{enali}}
\newcommand{\HC}[1][\scad]{\beaunom[#1]{Herv\'e}{C}{arfantan}}
\newcommand{\HS}[1][\scad]{\beaunom[#1]{Hichem}{S}{noussi}}
\newcommand{\JBP}[1][\scad]{\beaunom[#1]{Jean--Baptiste}{P}{oline}}
\newcommand{\JFB}[1][\scad]{\beaunom[#1]{Jean--Fran\c{c}ois}{B}{ercher}}
\newcommand{\JFG}[1][\scad]{\beaunom[#1]{Jean--Fran\c{c}ois}{G}{iovannelli}}
\newcommand{\JFM}[1][\scad]{\beaunom[#1]{Jean--Fran\c{c}ois}{M}{angin}}
\newcommand{\JJF}[1][\scad]{\beaunom[#1]{Jean--Jacques}{F}{uchs}}
\newcommand{\IB}[1][\scad]{\beaunom[#1]{Isabelle}{B}{loch}}
\newcommand{\JI}[1][\scad]{\beaunom[#1]{J\'er\^ome}{I}{dier}}
\newcommand{\JM}[1][\scad]{\beaunom[#1]{J\'er\'emie}{M}{attout}}
\newcommand{\JP}[1][\scad]{\beaunom[#1]{J\'er\'emie}{P}{escatore}}
\newcommand{\JPL}[1][\scad]{\beaunom[#1]{Jean--Philippe}{L}{achaux}}
\newcommand{\LG}[1][\scad]{\beaunom[#1]{Line}{G}{arnero}}
\newcommand{\LR}[1][\scad]{\beaunom[#1]{Laurent}{R}{isser}}
\newcommand{\MA}[1][\scad]{\beaunom[#1]{Marc}{A}{llain}}
\newcommand{\MF}[1][\scad]{\beaunom[#1]{Marc}{F}{ayolle}}
\newcommand{\Mimi}[1][\scad]{\beaunom[#1]{Myriam}{F}{iani}}
\newcommand{\MN}[1][\scad]{\beaunom[#1]{Mila}{N}{ikolova}}
\newcommand{\NaG}[1][\scad]{\beaunom[#1]{Nathalie}{G}{eorge}}
\newcommand{\NF}[1][\scad]{\beaunom[#1]{Nicole}{F}{iori}}
\newcommand{\NL}[1][\scad]{\beaunom[#1]{Nicolas}{L}{ori}}
\newcommand{\PC}[1][\scad]{\beaunom[#1]{Philippe}{C}{iuciu}}
\newcommand{\PF}[1][\scad]{\beaunom[#1]{Patrick}{F}{landrin}}
\newcommand{\PH}[1][\scad]{\beaunom[#1]{Philippe}{H}{entraye}}
\newcommand{\SB}[1][\scad]{\beaunom[#1]{St\'ephane}{B}{rette}}
\newcommand{\SBA}[1][\scad]{\beaunom[#1]{Sylvain}{B}{aillet}}
\newcommand{\SM}[1][\scad]{\beaunom[#1]{Salima}{M}{akni}}
\newcommand{\StD}[1][\scad]{\beaunom[#1]{Stanislas}{D}{ehaene}}
\newcommand{\RB}[1][\scad]{\beaunom[#1]{Redha}{B}{oubertakh}}
\newcommand{\RM}[1][\scad]{\beaunom[#1]{Renaud}{M}{aroy}}
\newcommand{\TL}[1][\scad]{\beaunom[#1]{Thomas}{L}{amotte}}
\newcommand{\TM}[1][\scad]{\beaunom[#1]{Thierry}{M}{artin}}
\newcommand{\TV}[1][\scad]{\beaunom[#1]{Thomas}{V}{incent}}
\newcommand{\VS}[1][\scad]{\beaunom[#1]{Vincent}{S}{amson}}
\newcommand{\VP}[1][\scad]{\beaunom[#1]{Viviane}{P}{outhas}}
\newcommand{\YB}[1][\scad]{\beaunom[#1]{Yves}{B}{urnod}}
\newcommand{\YC}[1][\scad]{\beaunom[#1]{Yann}{C}{ointepas}}
\newcommand{\YG}[1][\scad]{\beaunom[#1]{Yves}{G}{oussard}}
\newcommand{\KS}[1][\scad]{\beaunom[#1]{Ken}{S}{auer}}

% Acronymes et raccourcis
%
\def\ATER{Attach\'e temporaire d'enseignement et de recherche}
\newcommand{\ater}[1][\scad]{\sca[#1]{ater}\xspace}
\def\ADDOC{Agir pour les Doctorants et les jeunes Docteurs\XS}
\newcommand{\addoc}[1][\scad]{\sca[#1]{addoc}\XS}

%%%%Institutions %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CNRS, UFR, ...
\def\CNRS{Centre National de la Recherche Scientifique\XS}
\newcommand{\cnrs}[1][\scad]{\sca[#1]{cnrs}\XS}
\def\INRIA{Institut National de la Recherche en Informatique et en Automatique\XS}
\newcommand{\inria}[1][\scad]{\sca[#1]{inria}\XS}
\def\UFR{Unit\'e de Formation et de Recherche}
\newcommand{\ufr}[1][\scad]{\sca[#1]{ufr}\XS}
\def\CdO{Centre d'Orsay\XS}
% Universites
\def\UPS{Universit\'e de Paris--Sud\XS}
\newcommand{\ups}[1][\scad]{\sca[#1]{ups}\XS}
\newcommand{\upxi}[1][\scad]{\sca[#1]{upxi}\XS}
\def\UPVI{Universit\'e Paris~VI\XS}
\newcommand{\upvi}[1][\scad]{\sca[#1]{upvi}\XS}
\def\UPMC{Universit\'e Pierre et Marie Curie\XS}
\def\UMV{Universit\'e de Marne la Vall\'ee\XS}
\newcommand{\umv}[1][\scad]{\sca[#1]{umv}\XS}
\def\CNU{Conseil National des Universit\'es\XS}
\newcommand{\cnu}[1][\scad]{\sca[#1]{cnu}\XS}

% CEA, DSV, ...
\def\CEA{Commissariat \`a l'\'Energie Atomique\XS}
\newcommand{\cea}[1][\scad]{\sca[#1]{cea}\XS}
\newcommand{\dam}[1][\scad]{\sca[#1]{dam}\XS}
\def\DRM{D\'epartement de Recherche M\'edicale\XS}
\newcommand{\drm}[1][\scad]{\sca[#1]{drm}\XS}
\def\DSV{Direction des Sciences du Vivant\XS}
\newcommand{\dsv}[1][\scad]{\sca[#1]{dsv}\XS}
\newcommand{\leti}[1][\scad]{\sca[#1]{leti}\XS}
\def\SHFJ{Service Hospitalier Fr\'ed\'eric Joliot\XS}
\newcommand{\shfj}[1][\scad]{\sca[#1]{shfj}\XS}
\def\UNAF{Unit\'e de Neuro-imagerie Anatomo-Fonctionnelle\XS}
\newcommand{\unaf}[1][\scad]{\sca[#1]{unaf}\XS}
\def\LNAO{Laboratoire de Neuro-imagerie  Assist\'ee par Ordinateur\XS}
\newcommand{\lnao}[1][\scad]{\sca[#1]{lnao}\XS}
\def\MAD{Mod\`eles et Analyse de Donn\'ees\XS}
\newcommand{\uiibp}[1][\scad]{\sca[#1]{uiibp}\XS}
\newcommand{\mad}[1][\scad]{\sca[#1]{mad}\XS}
\def\IFR{Institut F\'ed\'eratif de Recherche\XS}
\newcommand{\ifr}[1][\scad]{\sca[#1]{ifr}\XS}
\def\STIC{Sciences et Technologies de l'Information et de la Communication\XS}
\newcommand{\stic}[1][\scad]{\sca[#1]{stic}\XS}
%INSERM
\def\INSERM{Institut National pour la Sant\'e et la Recherche M\'edicale\XS}
\newcommand{\inserm}[1][\scad]{\sca[#1]{inserm}\XS}
\def\UNICOG{Unit\'e de Neuroimagerie Cognitive\XS}
\newcommand{\unicog}[1][\scad]{\sca[#1]{unicog}\XS}
\newcommand{\ipsn}[1][\scad]{\sca[#1]{ipsn}\XS}
\def\IPSN{Institut de Protection et de Suret\'e Nucl\'eaire\XS}
%ONERA
\def\ONERA{Office National d'\'Etudes et de Recherches A\'erospatiales\XS}
\newcommand{\onera}[1][\scad]{\sca[#1]{on\'era}\XS}
\def\SAFC{Soci\'et\'e d'Anatomie Fonctionnelle C\'er\'ebrale\XS}
\newcommand{\safc}[1][\scad]{\sca[#1]{safc}\XS}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%% Labos, unit\'es, ...%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\chu}[1][\scad]{\sca[#1]{chu}\XS}
\def\CHU{Centre Hospitalier Universitaire\XS}
\def\salpe{Salp\'etri\'ere\XS}
\def\hsalpe{H\'epital de la Salp\'etri\'ere\XS}
\def\pisalpe{Piti\'e-Salp\'etri\'ere\XS}
\def\gpisalpe{Groupe Piti\'e-Salp\'etri\'ere\XS}
% Unite propre de recherche
\newcommand{\upr}[1][\scad]{\sca[#1]{upr}\XS}
\newcommand{\ura}[1][\scad]{\sca[#1]{ura}\XS}
% LENA, lena upr640,...
\newcommand{\lena}[1][\scad]{\sca[#1]{lena}\XS}
\newcommand{\sxqt}[1][\scad]{\sca[#1]{{\normalsize 640}}\XS}
\newcommand{\uprlen}[1][\scad]{\lena~--~\sca[#1]{upr}~\sxqt[#1]\XS}
\newcommand{\uprcnrs}[1][\scad]{\sca[#1]{upr}\,--\,\cnrs[#1]~{\small 640}\XS}
\newcommand{\uprs}[1][\scad]{\sca[#1]{upr}~{\small 640}\XS}
\newcommand{\uprss}[1][\scad]{\sca[#1]{upr}~--~\cnrs[#1]~\sxqt[#1]\XS}
%\newcommand{\uprs}[1][\scad]{\sca[#1]{UPR}~--~\cnrs[#1]~640\XS}

\newcommand{\lenatut}[1][\scad]{\cnrs[#1]~--~\upvi[#1]}
%\def\LENA{Laboratoire d'Enc\'ephalographie et de Neurophysiologie Appliqu\'ee\XS}
\def\LENA{Laboratoire de Neurosciences Cognitives et d'Imagerie C\'er\'ebrale\XS}
% def equipe Imagerie cerebrale
\def\TDIC{Traitement de Donn\'ees en Imagerie C\'er\'ebrale\XS}
\newcommand{\tdic}[1][\scad]{\sca[#1]{tdic}\XS}
\def\ADN{Analyse Dynamique Non lin\'eaire\XS}
\newcommand{\adn}[1][\scad]{\sca[#1]{adn}\XS}
%% labos \'e"trangers
\def\SIPI{Signal and Image Processing Institute\XS}
\newcommand{\sipi}[1][\scad]{\sca[#1]{sipi}\XS}
\def\USC{Universit\'e de Californie du Sud\XS}
\newcommand{\usc}[1][\scad]{\sca[#1]{usc}\XS}
\def\FIL{Functional Imaging Laboratory\XS}
\newcommand{\fil}[1][\scad]{\sca[#1]{fil}\XS}
\def\GPI{Groupe Probl\`emes Inverses\XS}
\newcommand{\gpi}[1][\scad]{\sca[#1]{gpi}\XS}
\def\IAS{Institut d'Astrophysique Spatiale\XS}
\newcommand{\ias}[1][\scad]{\sca[#1]{ias}\XS}
\def\LSS{Laboratoire des Signaux et Syst\`emes\XS}
\newcommand{\lss}[1][\scad]{\sca[#1]{l{\footnotesize 2}s}\XS}
\def\LIMSI{Laboratoire d'Informatique pour la M\'ecanique et les Sciences de l'Ing\'enieur\XS}
\newcommand{\limsi}[1][\scad]{\sca[#1]{limsi}\XS}
\def\LSCP{Laboratoire des Sciences Cognitives et Psycholinguistique\XS}
\newcommand{\lscp}[1][\scad]{\sca[#1]{lscp}\XS}
\def\EHESS{\'Ecole des Hautes \'Etudes en Sciences Sociales\XS}
\newcommand{\ehess}[1][\scad]{\sca[#1]{ehess}\XS}
\def\MRCCBU{MRC Cognition and Brain Sciences Unit\XS}
\newcommand{\mrccbu}[1][\scad]{\sca[#1]{mrc-cbu}\XS}
\def\IRCCYN{Institut de recherche en communications et en cybern\'etique de Nantes\XS}
\newcommand{\irccyn}[1][\scad]{\sca[#1]{irccyn}\XS}

\def\EDSTICS{\'Ecole Doctorale Sciences et Technologies de l'Information, de la Communication et des Syst\'emes.\XS}
\newcommand{\edstics}[1][\scad]{\sca[#1]{ed stics}\XS}
\def\FMRIB{\emph{Oxford Centre for Functional Magnetic Resonance Imaging of the Brain}\XS}
 \newcommand{\fmrib}[1][\scad]{\sca[#1]{Fmrib}\XS}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%Ecoles %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\ULP{Universit\'e Louis Pasteur, Strasbourg\XS}
\newcommand{\ulp}[1][\scad]{\sca[#1]{ulp}\XS}
%%%%%%%Ecoles %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\ENSPS{\'Ecole Nationale Sup\'erieure de Physique de Strasbourg\XS}
\newcommand{\ensps}[1][\scad]{\sca[#1]{ensps}\XS}
\def\ENSPM{\'Ecole Nationale Sup\'erieure de Physique\\[.5cm] de Marseille\XS}
\newcommand{\enspm}[1][\scad]{\sca[#1]{enspm}\XS}
\def\ENSL{\'Ecole Normale Sup\'erieure de Lyon\XS}
\newcommand{\ensl}[1][\scad]{\sca[#1]{ens} de Lyon\XS}
\def\ENSTA{\'Ecole Nationale Sup\'erieure de Techniques Avanc\'ees\XS}
\newcommand{\ensta}[1][\scad]{\sca[#1]{ensta}\XS}
\def\ESIEA{\'Ecole Sup\'erieure d'Informatique \'Electronique Automatique\XS}
\newcommand{\esiea}[1][\scad]{\sca[#1]{esiea}\XS}
\newcommand{\ensea}[1][\scad]{\sca[#1]{ensea}\XS}
\def\ENST{\'Ecole Nationale Sup\'erieure des T\'el\'ecommunications\XS}
\newcommand{\enst}[1][\scad]{\sca[#1]{enst}\XS}
\def\EPFL{\'Ecole Polytechnique F\'ed\'erale de Lausanne\XS}
\newcommand{\epfl}[1][\scad]{\sca[#1]{epfl}\XS}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\EVI{\emph{Echo Volumar Imaging}\XS}
\newcommand{\evi}[1][\scad]{\sca[#1]{evi}\XS}
\def\EPI{\emph{Echo Planar Imaging}\XS}
\newcommand{\epi}[1][\scad]{\sca[#1]{epi}\XS}


%%%%%%%Entreprises %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\edf}[1][\scad]{\sca[#1]{edf}\XS}
\def\EDF{\'Electricit\'e de France\XS}
% Unites Thomson
\newcommand{\thomair}[1][\scad]{\sca[#1]{Thomson-csf Airsys}\XS}
\newcommand{\oscar}[1][\scad]{\sca[#1]{Oscar}\XS}
\newcommand{\thomrcm}[1][\scad]{\sca[#1]{Thomson-rcm}\XS}
%\def\thomair{\textsc{Thomson--airsys}\XS}
%\def\thomrcm{\textsc{Thomson--rcm}\XS}
\newcommand{\rdran}[1][\scad]{\sca[#1]{rdran}\XS}
\newcommand{\rdta}[1][\scad]{\sca[#1]{rdta}\XS}
\newcommand{\thales}[1][\scad]{\sca[#1]{Thal\'es}\XS}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\MDC{Ma\^\i tre de conf\'erences\XS}
\def\MDCs{Ma\^\i tres de conf\'erences\XS}
\newcommand{\mdc}[1][\scad]{\sca[#1]{mdc}\XS}


% Adresse : LSS, SHFJ, ...
\def\GsY{Gif--sur--Yvette\XS}
\newcommand{\ESE}[1][\scad]{\sca[#1]{sup\'elec}\XS}
\def\adrshort{\ESE, Plateau de Moulon, 91192 Gif--sur--Yvette Cedex\XS}
%\def\adresse{\ESE, Plateau de Moulon, 91192 Gif--sur--Yvette Cedex, France\XS}
%\newcommand{\adresse}[1][\scad]{\ESE[#1], Plateau de Moulon, 91192 Gif--sur--Yvette Cedex, France\XS}
\newcommand{\tutelle}[1][\scad]{\cnrs[#1]~--~\ESE[#1]~--~\ups[#1]}
\newcommand{\hiercea}[1][\scad]{\dsv[#1]/\drm[#1]/\shfj[#1]}
%\newcommand{\tutelle}[1][\scad]{\sca[#1]{Cnrs~--~Sup\'elec~--~Ups}}
%\def\ALSS{\LSS~(\tutelle)\\\adresse}
%\def\ALSSun{\LSS (\tutelle) \adresse}
\newcommand{\adresscea}[1][\scad]{4 Place du G\'en\'eral Leclerc, 91406 Orsay Cedex, France\XS}
% ---------------------------------------------------- 
% Modele d'en-tete par A. Mohammad-Djafari et J. Idier 
% ---------------------------------------------------- 
%
\def\helvnormal#1{{\fontfamily{phv}\fontsize{11}{14pt}\selectfont #1}}
\def\helvfoot  #1{{\fontfamily{phv}\fontsize{9}{14pt} \selectfont #1}}
\def\helvscript#1{{\fontfamily{phv}\fontsize{8}{14pt} \selectfont #1}}
%
\newcommand{\entete}[5][Nom.Pr\'enom]{
%%%%%%\def\entete#1#2#3#4#5
\helvscript{\renewcommand{\arraystretch}{.8}
\begin{tabular}{c} Sup\'elec
\\--------\end{tabular} \hfill
\begin{tabular}{c}Centre national de la recherche scientifique          \\
--------\end{tabular} \hfill
\begin{tabular}{c}\UPS  \\--------\end{tabular}} \\[-.4cm]%
%
\begin{center}\helvnormal{\textbf{LABORATOIRE DES SIGNAUX \& SYST\`EMES}}\\%
\helvfoot{Unit\'e mixte de recherche n$^{\rm o}$ 8506\\%
Sup\'elec, plateau de Moulon, 
3 rue Joliot-Curie, 91192 \sca[-3]{Gif--sur--Yvette} Cedex (France)\\%
T\'el\'ephone\,: 01 69 85 17 12 --- 
T\'el\'ecopie\,: 01 69 85 17 65 --- 
Courriel\,: {#1}@lss.supelec.fr}%
\\[0.5cm]\end{center}% 
\begin{tabular}{p{8.5cm}l}%
\helvscript{V/R\'ef.\,: #2} & \helvscript{\sca[-3]{Gif}, le} #5\\%
\helvscript{N/R\'ef.\,: #3} \\%
\helvscript{Objet\,: #4}%
\end{tabular}
}

\newcommand{\inhead}[5][Name.Surname]{
%%%%%%\def\entete#1#2#3#4#5
\helvscript{\renewcommand{\arraystretch}{.8}
\begin{tabular}{c} Sup\'elec
\\--------\end{tabular} \hfill
\begin{tabular}{c}Centre national de la recherche scientifique  \\
--------\end{tabular} \hfill
\begin{tabular}{c}\UPS  \\--------\end{tabular}} \\[-.4cm]%
%
\begin{center}\helvnormal{\textbf{LABORATOIRE DES SIGNAUX \& SYST\`EMES}}\\%
\helvfoot{Unit\'e mixte de recherche n$^{\rm o}$ 8506\\%
Sup\'elec, plateau de Moulon, 
3 rue Joliot-Curie, 91192 \sca[-3]{Gif--sur--Yvette} Cedex (France)\\%
Telephone: (33)-1 69 85 17 12 --- 
Fax: (33)-1 69 85 17 65 --- 
E-mail: {#1}@lss.supelec.fr}%
\\[0.5cm]\end{center}% 
\begin{tabular}{p{8.5cm}l}%
\helvscript{Y/Ref.: #2} & \helvscript{\sca[-3]{Gif}, } #5\\%
\helvscript{O/Ref.: #3} \\%
\helvscript{Subject: #4}%
\end{tabular}
}

%Direction des Sciences du Vivant/
%\helvfoot{D\'epartement de la Recherche M\'edicale\\%
%Service Hospitalier Fr\'ed\'eric Joliot, 4 place du g\'en\'eral Leclerc,
%91406 \sca[-3]{Orsay} (France)\\%
%T\'el\'ephone\,: #6 --- T\'el\'ecopie\,: 01 69 86 77 86 ---
%Courriel\,: {#1}@shfj.cea.fr}%
%\helvfoot{T\'el\'ephone\,: {#6} --- T\'el\'ecopie\,: 01 69 86 77 86 --- Courriel\,: {#1}@shfj.cea.fr}

\newcommand{\entetecea}[6][prenom.nom]{
%%%%%%\def\entetecea#1#2#3#4#5#6
\begin{center}\helvnormal{\textbf{COMMISSARIAT \`A l'\'ENERGIE ATOMIQUE}}\\%
\helvfoot{Direction des Sciences du Vivant/D\'epartement de la Recherche M\'edicale}\\
\helvfoot{Service Hospitalier Fr\'ed\'eric Joliot, 4 place du g\'en\'eral Leclerc,
91406 \sca[-3]{Orsay} (France)}\\
\helvfoot{T\'el\'ephone : 01 69 86 78 67 --- T\'el\'ecopie : 01 69 86 77 86 --- Courriel\,: {#1}@cea.fr}\\[0.5cm]
\end{center}% 
\begin{tabular}{p{8.5cm}l}%
\helvscript{V/R\'ef.\,: #2} & \helvscript{\sca[-3]{Orsay}, le} #5\\%
\helvscript{N/R\'ef.\,: #3} \\%
\helvscript{Objet\,: #4}%
\end{tabular}
} 

\newcommand{\inheadcea}[6][firstname.lastname]{
%%%%%%\def\inheadcea#1#2#3#4#5#6
\begin{center}\helvnormal{\textbf{COMMISSARIAT \`A l'\'ENERGIE ATOMIQUE}}\\%
\helvfoot{Life Science Division/Medical research department}\\%
\helvfoot{Service Hospitalier Fr\'ed\'eric Joliot, 4 place du g\'en\'eral Leclerc,
91406 \sca[-3]{Orsay} (France)}\\
\helvfoot{Phone: (33) 1 69 86 78 67 --- Fax: (33) 1 69 86 77 86 --- E-mail: {#1}@cea.fr}\\[0.5cm]
\end{center}% 
\begin{tabular}{p{8.5cm}l}%
\helvscript{Y/Ref.: #2} & \helvscript{\sca[-3]{Orsay}, } #5\\%
\helvscript{O/Ref.: #3} \\%
\helvscript{Subject: #4}%
\end{tabular}
} 

\newcommand{\enteteneurospin}[6][prenom.nom]{
%%%%%%\def\entetecea#1#2#3#4#5#6
\begin{center}
\helvnormal{\textbf{COMMISSARIAT \`A l'\'ENERGIE ATOMIQUE}}\\%
\helvfoot{Direction des Sciences du Vivant/Institut d'imagerie biom\'edicale}\\
\helvfoot{NeuroSpin, B\^atiment 145 -- Point Courrier 156, CEA Saclay
91191 \sca[-3]{Gif-sur-Yvette} cedex (France)}\\
\helvfoot{T\'el\'ephone : 01 69 08 77 85 --- T\'el\'ecopie : 01 69 08 79 80 --- Courriel\,: {#1}@cea.fr}\\[0.5cm]
\end{center}% 
\begin{tabular}{p{8.5cm}l}%
\helvscript{V/R\'ef.\,: #2} & \helvscript{\sca[-3]{Gif-sur-Yvette}, le} #5\\%
\helvscript{N/R\'ef.\,: #3} \\%
\helvscript{Objet\,: #4}%
\end{tabular}
} 

\newcommand{\inheadneurospin}[6][prenom.nom]{
%%%%%%\def\entetecea#1#2#3#4#5#6
\begin{center}\helvnormal{\textbf{COMMISSARIAT \`A l'\'ENERGIE ATOMIQUE}}\\%
\helvfoot{Life Science Division/Biomedical Imaging Institute}\\
\helvfoot{NeuroSpin, B\^atiment 145 -- Point Courrier 156, CEA Saclay
91191 \sca[-3]{Gif-sur-Yvette} cedex (France)}\\
\helvfoot{Phone : 01 69 08 77 85 --- Fax : 01 69 08 79 80 --- e-mail\,: {#1}@cea.fr}\\[0.5cm]
\end{center}% 
\begin{tabular}{p{8.5cm}l}%
\helvscript{V/R\'ef.\,: #2} & \helvscript{\sca[-3]{Gif-sur-Yvette}, le} #5\\%
\helvscript{N/R\'ef.\,: #3} \\%
\helvscript{Objet\,: #4}%
\end{tabular}
} 


==> alphabet.tex <==
% Document LaTeX        Auteur : Philippe Ciuciu      Date : 06/08/01
% Objet : Definitions compactes d'alphabets pour ecriture en Math
% b pour bold italique : \Ab
% v pour bold droit : \Av
% D pour droit : \AD
% c pour cursif : \Ac
% bb pour blackboard : \Abb
% Capitale pour capitale : \Lambda

\typeout{\space}
\typeout{\space\space\space\space Fichier 'alphabet.tex' -- SHFJ 2001}
\typeout{\space\space\space\space (necessite les packages xspace, amsmath, bbm)}
\typeout{\space}

\RequirePackage{amsmath}
\RequirePackage{xspace}
\RequirePackage{bbm}

%-------------------------------------------

% DEFINITIONS PRELIMINAIRES 

\def\XS{\xspace}
\DeclareMathAlphabet{\mathb}{OML}{cmm}{b}{it}
\def\sbm#1{\ensuremath{\mathb{#1}}}                % Style gras italique (necessite amsmath)           
%
\def\sbmm#1{\ensuremath{\boldsymbol{#1}}}          % Style gras italique (necessite amsmath)           
\def\sdm#1{\ensuremath{\mathrm{#1}}}               % Style droit en math
\def\sbv#1{\ensuremath{\mathbf{#1}}}               % Style gras droit
\def\scu#1{\ensuremath{\mathcal{#1\XS}}}           % Style cursif
\def\scb#1{\ensuremath{\boldsymbol{\mathcal{#1}}}} % Style gras cursif
\def\sbl#1{\ensuremath{\mathbbm{#1}}}              % Style blackboard (necessite bbm)

%-------------------------------------------

% ALPHABET GRAS ITALIQUE, taille adaptative

\def\Ab{{\sbm{A}}\XS}  \def\ab{{\sbm{a}}\XS}
\def\Bb{{\sbm{B}}\XS}  \def\bb{{\sbm{b}}\XS}
\def\Cb{{\sbm{C}}\XS}  \def\cb{{\sbm{c}}\XS}
\def\Db{{\sbm{D}}\XS}  \def\db{{\sbm{d}}\XS}
\def\Eb{{\sbm{E}}\XS}  \def\eb{{\sbm{e}}\XS}
\def\Fb{{\sbm{F}}\XS}  \def\fb{{\sbm{f}}\XS}
\def\Gb{{\sbm{G}}\XS}  \def\gb{{\sbm{g}}\XS}
\def\Hb{{\sbm{H}}\XS}  \def\hb{{\sbm{h}}\XS}
\def\Ib{{\sbm{I}}\XS}  \def\ib{{\sbm{i}}\XS}
\def\Jb{{\sbm{J}}\XS}  \def\jb{{\sbm{j}}\XS}
\def\Kb{{\sbm{K}}\XS}  \def\kb{{\sbm{k}}\XS}
\def\Lb{{\sbm{L}}\XS}  \def\lb{{\sbm{l}}\XS}
\def\Mb{{\sbm{M}}\XS}  \def\mb{{\sbm{m}}\XS}
\def\Nb{{\sbm{N}}\XS}  \def\nb{{\sbm{n}}\XS}
\def\Ob{{\sbm{O}}\XS}  \def\ob{{\sbm{o}}\XS}
\def\Pb{{\sbm{P}}\XS}  \def\pb{{\sbm{p}}\XS}
\def\Qb{{\sbm{Q}}\XS}  \def\qb{{\sbm{q}}\XS}
\def\Rb{{\sbm{R}}\XS}  \def\rb{{\sbm{r}}\XS}
\def\Sb{{\sbm{S}}\XS}  \def\sb{{\sbm{s}}\XS}
\def\Tb{{\sbm{T}}\XS}  \def\tb{{\sbm{t}}\XS}
\def\Ub{{\sbm{U}}\XS}  \def\ub{{\sbm{u}}\XS}
\def\Vb{{\sbm{V}}\XS}  \def\vb{{\sbm{v}}\XS}
\def\Wb{{\sbm{W}}\XS}  \def\wb{{\sbm{w}}\XS}
\def\Xb{{\sbm{X}}\XS}  \def\xb{{\sbm{x}}\XS}
\def\Yb{{\sbm{Y}}\XS}  \def\yb{{\sbm{y}}\XS}
\def\Zb{{\sbm{Z}}\XS}  \def\zb{{\sbm{z}}\XS}


% ALPHABET CURSIF MAJUSCULE, taille adaptative
% Cursif,               % Cursif gras

\def\Ac{{\scu{A}}\XS}   \def\Acb{{\scb{A}}\XS}
\def\Bc{{\scu{B}}\XS}   \def\Bcb{{\scb{B}}\XS}
\def\Cc{{\scu{C}}\XS}   \def\Ccb{{\scb{C}}\XS}
\def\Dc{{\scu{D}}\XS}   \def\Dcb{{\scb{D}}\XS}
\def\Ec{{\scu{E}}\XS}   \def\Ecb{{\scb{E}}\XS}
\def\Fc{{\scu{F}}\XS}   \def\Fcb{{\scb{F}}\XS}
\def\Gc{{\scu{G}}\XS}   \def\Gcb{{\scb{G}}\XS}
\def\Hc{{\scu{H}}\XS}   \def\Hcb{{\scb{H}}\XS}
\def\Ic{{\scu{I}}\XS}   \def\Icb{{\scb{I}}\XS}
\def\Jc{{\scu{J}}\XS}   \def\Jcb{{\scb{J}}\XS}
\def\Kc{{\scu{K}}\XS}   \def\Kcb{{\scb{K}}\XS}
\def\Lc{{\scu{L}}\XS}   \def\Lcb{{\scb{L}}\XS}
\def\Mc{{\scu{M}}\XS}   \def\Mcb{{\scb{M}}\XS}
\def\Nc{{\scu{N}}\XS}   \def\Ncb{{\scb{N}}\XS}
\def\Oc{{\scu{O}}\XS}   \def\Ocb{{\scb{O}}\XS}
\def\Pc{{\scu{P}}\XS}   \def\Pcb{{\scb{P}}\XS}
\def\Qc{{\scu{Q}}\XS}   \def\Qcb{{\scb{Q}}\XS}
\def\Rc{{\scu{R}}\XS}   \def\Rcb{{\scb{R}}\XS}
\def\Sc{{\scu{S}}\XS}   \def\Scb{{\scb{S}}\XS}
\def\Tc{{\scu{T}}\XS}   \def\Tcb{{\scb{T}}\XS}
\def\Uc{{\scu{U}}\XS}   \def\Ucb{{\scb{U}}\XS}
\def\Vc{{\scu{V}}\XS}   \def\Vcb{{\scb{V}}\XS}
\def\Wc{{\scu{W}}\XS}   \def\Wcb{{\scb{W}}\XS}
\def\Xc{{\scu{X}}\XS}   \def\Xcb{{\scb{X}}\XS}
\def\Yc{{\scu{Y}}\XS}   \def\Ycb{{\scb{Y}}\XS}
\def\Zc{{\scu{Z}}\XS}   \def\Zcb{{\scb{Z}}\XS}


% ALPHABET DROIT EN MATHS, taille adaptative

\def\AD{{\sdm{A}}\XS}  \def\aD{{\sdm{a}}\XS}
\def\BD{{\sdm{B}}\XS}  \def\bD{{\sdm{b}}\XS}
\def\CD{{\sdm{C}}\XS}  \def\cD{{\sdm{c}}\XS}
\def\DD{{\sdm{D}}\XS}  \def\dD{{\sdm{d}}\XS}
\def\ED{{\sdm{E}}\XS}  \def\eD{{\sdm{e}}\XS}
\def\FD{{\sdm{F}}\XS}  \def\fD{{\sdm{f}}\XS}
\def\GD{{\sdm{G}}\XS}  \def\gD{{\sdm{g}}\XS}
\def\HD{{\sdm{H}}\XS}  \def\hD{{\sdm{h}}\XS}
\def\ID{{\sdm{I}}\XS}  \def\iD{{\sdm{i}}\XS}
\def\JD{{\sdm{J}}\XS}  \def\jD{{\sdm{j}}\XS}
\def\KD{{\sdm{K}}\XS}  \def\kD{{\sdm{k}}\XS}
\def\LD{{\sdm{L}}\XS}  \def\lD{{\sdm{l}}\XS}
\def\MD{{\sdm{M}}\XS}  \def\mD{{\sdm{m}}\XS}
\def\ND{{\sdm{N}}\XS}  \def\nD{{\sdm{n}}\XS}
\def\OD{{\sdm{O}}\XS}  \def\oD{{\sdm{o}}\XS}
\def\PD{{\sdm{P}}\XS}  \def\pD{{\sdm{p}}\XS}
\def\QD{{\sdm{Q}}\XS}  \def\qD{{\sdm{q}}\XS}
\def\RD{{\sdm{R}}\XS}  \def\rD{{\sdm{r}}\XS}
\def\SD{{\sdm{S}}\XS}  \def\sD{{\sdm{s}}\XS}
\def\TD{{\sdm{T}}\XS}  \def\tD{{\sdm{t}}\XS}
\def\UD{{\sdm{U}}\XS}  \def\uD{{\sdm{u}}\XS}
\def\VD{{\sdm{V}}\XS}  \def\vD{{\sdm{D}}\XS}
\def\WD{{\sdm{W}}\XS}  \def\wD{{\sdm{w}}\XS}
\def\XD{{\sdm{X}}\XS}  \def\xD{{\sdm{x}}\XS}
\def\YD{{\sdm{Y}}\XS}  \def\yD{{\sdm{y}}\XS}
\def\ZD{{\sdm{Z}}\XS}  \def\zD{{\sdm{z}}\XS}


% ALPHABET GRAS DROIT, taille adaptative

\def\Av{{\sbv{A}}\XS}  \def\av{{\sbv{a}}\XS}
\def\Bv{{\sbv{B}}\XS}  \def\bv{{\sbv{b}}\XS}
\def\Cv{{\sbv{C}}\XS}  \def\cv{{\sbv{c}}\XS}
\def\Dv{{\sbv{D}}\XS}  \def\dv{{\sbv{d}}\XS}
\def\Ev{{\sbv{E}}\XS}  \def\ev{{\sbv{e}}\XS}
\def\Fv{{\sbv{F}}\XS}  \def\fv{{\sbv{f}}\XS}
\def\Gv{{\sbv{G}}\XS}  \def\gv{{\sbv{g}}\XS}
\def\Hv{{\sbv{H}}\XS}  \def\hv{{\sbv{h}}\XS}
\def\Iv{{\sbv{I}}\XS}  \def\iv{{\sbv{i}}\XS}
\def\Jv{{\sbv{J}}\XS}  \def\jv{{\sbv{j}}\XS}
\def\Kv{{\sbv{K}}\XS}  \def\kv{{\sbv{k}}\XS}
\def\Lv{{\sbv{L}}\XS}  \def\lv{{\sbv{l}}\XS}
\def\Mv{{\sbv{M}}\XS}  \def\mv{{\sbv{m}}\XS}
\def\Nv{{\sbv{N}}\XS}  \def\nv{{\sbv{n}}\XS}
\def\Ov{{\sbv{O}}\XS}  \def\ov{{\sbv{o}}\XS}
\def\Pv{{\sbv{P}}\XS}  \def\pv{{\sbv{p}}\XS}
\def\Qv{{\sbv{Q}}\XS}  \def\qv{{\sbv{q}}\XS}
\def\Rv{{\sbv{R}}\XS}  \def\rv{{\sbv{r}}\XS}
\def\Sv{{\sbv{S}}\XS}  \def\sv{{\sbv{s}}\XS}
\def\Tv{{\sbv{T}}\XS}  \def\tv{{\sbv{t}}\XS}
\def\Uv{{\sbv{U}}\XS}  \def\uv{{\sbv{u}}\XS}
\def\Vv{{\sbv{V}}\XS}  \def\vv{{\sbv{v}}\XS}
\def\Wv{{\sbv{W}}\XS}  \def\wv{{\sbv{w}}\XS}
\def\Xv{{\sbv{X}}\XS}  \def\xv{{\sbv{x}}\XS}
\def\Yv{{\sbv{Y}}\XS}  \def\yv{{\sbv{y}}\XS}
\def\Zv{{\sbv{Z}}\XS}  \def\zv{{\sbv{z}}\XS}


% Nouveau (08/99) : ALPHABET BLACKBOARD, taille adaptative

\def\Abb{{\sbl{A}}\XS}  \def\abb{{\sbl{a}}\XS}
\def\Bbb{{\sbl{B}}\XS}  \def\bbb{{\sbl{b}}\XS}
\def\Cbb{{\sbl{C}}\XS}  \def\cbb{{\sbl{c}}\XS}
\def\Dbb{{\sbl{D}}\XS}  \def\dbb{{\sbl{d}}\XS}
\def\Ebb{{\sbl{E}}\XS}  \def\ebb{{\sbl{e}}\XS}
\def\Fbb{{\sbl{F}}\XS}  \def\fbb{{\sbl{f}}\XS}
\def\Gbb{{\sbl{G}}\XS}  \def\gbb{{\sbl{g}}\XS}
\def\Hbb{{\sbl{H}}\XS}  \def\hbb{{\sbl{h}}\XS}
\def\Ibb{{\sbl{I}}\XS}  \def\ibb{{\sbl{i}}\XS}
\def\Jbb{{\sbl{J}}\XS}  \def\jbb{{\sbl{j}}\XS}
\def\Kbb{{\sbl{K}}\XS}  \def\kbb{{\sbl{k}}\XS}
\def\Lbb{{\sbl{L}}\XS}  \def\lbb{{\sbl{l}}\XS}
\def\Mbb{{\sbl{M}}\XS}  \def\mbb{{\sbl{m}}\XS}
\def\Nbb{{\sbl{N}}\XS}  \def\nbb{{\sbl{n}}\XS}
\def\Obb{{\sbl{O}}\XS}  \def\obb{{\sbl{o}}\XS}
\def\Pbb{{\sbl{P}}\XS}  \def\pbb{{\sbl{p}}\XS}
\def\Qbb{{\sbl{Q}}\XS}  \def\qbb{{\sbl{q}}\XS}
\def\Rbb{{\sbl{R}}\XS}  \def\rbb{{\sbl{r}}\XS}
\def\Sbb{{\sbl{S}}\XS}  \def\sbb{{\sbl{s}}\XS}
\def\Tbb{{\sbl{T}}\XS}  \def\tbb{{\sbl{t}}\XS}
\def\Ubb{{\sbl{U}}\XS}  \def\ubb{{\sbl{u}}\XS}
\def\Vbb{{\sbl{V}}\XS}  \def\vbb{{\sbl{v}}\XS}
\def\Wbb{{\sbl{W}}\XS}  \def\wbb{{\sbl{w}}\XS}
\def\Xbb{{\sbl{X}}\XS}  \def\xbb{{\sbl{x}}\XS}
\def\Ybb{{\sbl{Y}}\XS}  \def\ybb{{\sbl{y}}\XS}
\def\Zbb{{\sbl{Z}}\XS}  \def\zbb{{\sbl{z}}\XS}


% ALPHABET GREC GRAS, taille adaptative

\def\alphab      {{\sbmm{\alpha}}\XS}
\def\betab       {{\sbmm{\beta}}\XS}
\def\gammab      {{\sbmm{\gamma}}\XS}      \def\Gammab    {{\sbmm{\Gamma}}\XS}
\def\deltab      {{\sbmm{\delta}}\XS}      \def\Deltab    {{\sbmm{\Delta}}\XS}
\def\epsilonb    {{\sbmm{\epsilon}}\XS}
\def\varepsilonb {{\sbmm{\varepsilon}}\XS}
\def\etab        {{\sbmm{\eta}}\XS}
\def\thetab      {{\sbmm{\theta}}\XS}      \def\Thetab    {{\sbmm{\Theta}}\XS}
\def\varthetab   {{\sbmm{\vartheta}}\XS}
\def\iotab       {{\sbmm{\iota}}\XS}
\def\kappab      {{\sbmm{\kappa}}\XS}
\def\lambdab     {{\sbmm{\lambda}}\XS}    \def\Lambdab   {{\sbmm{\Lambda}}\XS}
\def\mub         {{\sbmm{\mu}}\XS}
\def\nub         {{\sbmm{\nu}}\XS}
\def\xib         {{\sbmm{\xi}}\XS}                 \def\Xib        {{\sbmm{\Xi}}\XS}
\def\pib         {{\sbmm{\pi}}\XS}                 \def\Pib        {{\sbmm{\Pi}}\XS}
\def\varpib      {{\sbmm{\varpi}}\XS}
\def\rhob        {{\sbmm{\rho}}\XS}
\def\varrhob     {{\sbmm{\varrho}}\XS}
\def\sigmab      {{\sbmm{\sigma}}\XS}      \def\Sigmab    {{\sbmm{\Sigma}}\XS}
\def\varsigmab   {{\sbmm{\varsigma}}\XS}  \def\Varsigmab {{\sbmm{\Varsigma}}\XS}
\def\phib        {{\sbmm{\phi}}\XS}        \def\Phib       {{\sbmm{\Phi}}\XS}
\def\varphib     {{\sbmm{\varphi}}\XS}
\def\chib        {{\sbmm{\chi}}\XS}
\def\psib        {{\sbmm{\psi}}\XS}        \def\Psib       {{\sbmm{\Psi}}\XS}
\def\omegab      {{\sbmm{\omega}}\XS}      \def\Omegab    {{\sbmm{\Omega}}\XS}
\def\taub        {{\sbmm{\tau}}\XS}
\def\upsilonb    {{\sbmm{\upsilon}}\XS}   \def\Upsilonb  {{\sbmm{\Upsilon}}\XS}
\def\zetab       {{\sbmm{\zeta}}\XS}


% CHIFFRES
% Gras et Blackboard, taille adaptative

\def\zerob   {{\sbv{0}}\XS}        \def\zerobb   {{\sbl{O}}\XS}
\def\unb     {{\sbv{1}}\XS}        \def\unbb     {{\sbl{1}}\XS}
\def\deuxb   {{\sbv{2}}\XS}        \def\deuxbb   {{\sbl{2}}\XS}
\def\troisb  {{\sbv{3}}\XS}        \def\troisbb  {{\sbl{3}}\XS}
\def\quatreb {{\sbv{4}}\XS}        \def\quatrebb {{\sbl{4}}\XS}
\def\cinqb   {{\sbv{5}}\XS}        \def\cinqbb   {{\sbl{5}}\XS}
\def\sixb    {{\sbv{6}}\XS}        \def\sixbb    {{\sbl{6}}\XS}
\def\septb   {{\sbv{7}}\XS}        \def\septbb   {{\sbl{7}}\XS}
\def\huitb   {{\sbv{8}}\XS}        \def\huitbb   {{\sbl{8}}\XS}
\def\neufb   {{\sbv{9}}\XS}        \def\neufbb   {{\sbl{9}}\XS}


% QUELQUES ENSEMBLES

\def\eC{\Cbb}
\def\eE{\Ebb}
\def\eN{\Nbb}
\def\eQ{\Qbb}
\def\eR{\Rbb}
\def\eZ{\Zbb}

\def\ellb{\sbmm{\ell}\XS} 


